Enabling Incremental Knowledge Transfer for Object Detection at the Edge

Object detection using deep neural networks (DNNs) involves a huge amount of computation which impedes its implementation on resource/energy-limited user-end devices. The reason for the success of DNNs is due to having knowledge over all different domains of observed environments. However, we need a limited knowledge of the observed environment at inference time which can be learned using a shallow neural network (SHNN). In this paper, a system-level design is proposed to improve the energy consumption of object detection on the user-end device. An SHNN is deployed on the user-end device to detect objects in the observing environment. Also, a knowledge transfer mechanism is implemented to update the SHNN model using the DNN knowledge when there is a change in the object domain. DNN knowledge can be obtained from a powerful edge device connected to the user-end device through LAN or Wi-Fi. Experiments demonstrate that the energy consumption of the user-end device and the inference time can be improved by 78% and 71% compared with running the deep model on the user-end device.

==> Introduction.tex <==
\section{Introduction}
\label{intro}

\begin{figure}[t!]
    \centering
    \includegraphics[trim=4.8cm 3.0cm 4cm 1.7cm, clip=true,width=9.0cm]{./images/KT2.pdf}
    %\vspace{-5}
    \caption{The limited knowledge of shallow model can be adapted to the new environment using the deep model knowledge.}
    \label{motivation}
\end{figure}

In the era of IoT (Internet of Things), miniaturized devices with sensing, computation, and communication capabilities have been utilized in embedded system. These embedded systems are used in a diverse set of applications such as surveillance, retail, and autonomous systems. 

In such applications, the the user-end device (i.e. the first recipient of camera frames) needs to identify and detect the objects in the scene in a timely manner. Object detection using Convolutional Neural Networks (CNNs) have gained attention which has led researchers to delve into deep models such as RetinaNet \cite{lin2017focal} and Faster-RCNN \cite{ren2015faster}. These models can achieve higher accuracy by stacking up several repetitive layers of convolution. The usage of deeper models opens up the opportunity of learning to detect a wider domain of objects which is time consuming and energy demanding.


Therefore, the user-end device with the limitation of computation and/or energy resources may not be able to run the deep detection models with reasonable response time. One possible solution would be to use a cloud server to face with the resource limitation of user-end devices.    

The studies in \cite{mao2019mobieye,chen2015glimpse} have used a cloud server for object detection along with a tracking method on the user-end device. However, this approach suffers from high response time for the newly observed objects in the scene. This is due to the fact that sending the camera frames to a cloud server starts to become infeasible because of high network latency and bandwidth limitation in IoT era. Moreover, using a cloud server may have serious challenges of preserving the security. 

Edge computing has been proposed to solve the mentioned issues by having a part or all of the computation on an edge device connected to the user-end device via a Local Area Connection (LAN) or Wi-Fi connection. Indeed, processing all the frames on the edge device will lead to high response time due to the large amount of input data being transmitted over the communication network.    

On the other hand, object detection methods mainly do not consider that a limited domain of objects is being observed in real-world applications \cite{farhadi2019tkd}. Thus, we may not need a deep model to learn this limited domain of objects. 

The limited domain of objects usually changes with a slow pace. Hence, a shallow model can be adapted to these changes whenever it is required. The knowledge of these changes can be gained from a deep model (Figure \ref{motivation}) and transferred to a shallow model using knowledge distillation \cite{farhadi2019tkd,mullapudi2019online} at run-time inference. This knowledge transfer enables us to improve the inference time of object detection while maintaining the accuracy of deep model.  

In order to implement the proposed approach, the user-end device runs the shallow model while the deep model is executed on the edge device. At some key frames, the knowledge of the shallow model is updated using the deep model on the edge device via a communication medium (LAN or Wi-Fi). The parameters of the CNN in the decoder layers (layers that detect the objects using the extracted features from previous layers) hold this knowledge. 

We have implemented the proposed approach on a pair of devices where the user-end device is NVIDIA Jetson Nano kit and a Dell workstation with Titan Xp GPU is the edge device. It has been shown that the proposed method can achieve the desired accuracy while having a significantly lower inference time. It has been demonstrated that the total energy consumption of the user-end device was reduced by approximately 78\% when compared to running the deep model.     


The main contributions of this paper are listed as follow:
\begin{itemize}
    \item We open up the opportunity to transfer the knowledge from a deep model to a shallow one in edge computing domain. Additionally, an exhaustive study on different possible designs of knowledge transfer has been done.  
    \item A novel key frame selector has been designed to enhance the efficiency of knowledge transfer.
    \item We have also built an open-source framework for incremental learning in object detection methods. The source code is released on Github. 
    
\end{itemize}
The rest of this paper is organized as follows: Section \ref{related} summarizes the background and related work which has been done previously. In Section \ref{approach}, the proposed approach using edge computing has been proposed. The experimental platform and the results are illustrated in Section \ref{results}. Ultimately, the conclusions are drawn in Section \ref{conclusion}. 

==> Introduction_SV_v2.tex <==
\section{Introduction}
\label{intro}

The Internet of Things (IoT) refers to a world in which almost any \textit{thing} is instrumented with sensors, computers and and communication devices. These \textit{embedded} systems will be utilized in a wide range of domains including  surveillance, retail, healthcare, transportation and logistics, industrial robotics and many more. The emergence of IoT is taking place along with a radical change in how the captured data is processed, namely, with the use of deep neural networks (DNNs). They have become the dominant algorithmic framework for extracting valuable information from massive amounts of disparate data for the purpose of prediction, classification and ultimately decision making. DNNs are computationally intensive algorithms that involve 10s to 100s of layers of nodes that perform billions of floating point multiply-accumulate operations on very large dimensional data sets, and often involve million of parameters.  Consequently they have to be executed on high performance, large capacity cloud servers. Unfortunately, this means that the massive amounts of data generated by the millions (soon to be in the billions) of IoT devices needs to be transferred to cloud, which will soon make this approach infeasible due to the limited bandwidth, the unacceptably large latency, and the potential for compromising the security of data.  

The preferred solution is to have some or all the data processed by a \textit{user-end} device, which is the first recipient of the data (e.g. a smartphone or a smart camera deployed in a public space). However, the limited computation and storage capabilities and/or energy capacity of user-end devices precludes them from executing complex DNN algorithms.  Edge computing is aimed at addressing this problem by having a part or all of the computation performed on a more powerful local computer called an \textit{edge} device that is connected to the user-end device via a local area network (LAN) or WiFi connection.

In this paper, we present a new approach to improve the execution of DNN algorithms in an edge computing environment.  The proposed system targets complex DNN algorithms (e.g., RetinaNet~\cite{lin2017focal}, Faster-RCNN~\cite{ren2015faster}) designed for \textit{object detection} in digital images and videos. Object detection arises in practically every computer vision task and now plays a central role in nearly every one of the applications domains mentioned above. The goal of this work is to demonstrate how two devices~--~a lower performance user-end device and a much higher performance edge device  can cooperate in the execution of computationally intensive DNN algorithms to achieve substantial improvement in energy consumption of the user-end device while achieving nearly the same quality of results as would be if the algorithms were executed solely on the more powerful device.  

\begin{figure}[t]
    \centering
    \includegraphics[trim=5.3cm 7.2cm 4cm 1.7cm, clip=true,width=8.5cm]{./images/TKD2.pdf}
    \caption{The limited knowledge of shallow model can be adapted to the new environment using the deep model knowledge.}
    \label{motivation}
\end{figure}

The proposed approach is based on a two-level hierarchy of models~--~a \textit{shallow} neural network (SNN) (the \textit{student}) that runs on the user-end device, and a DNN (the \textit{teacher}) that runs on the more powerful edge device.  The edge device can also execute the SNN. The use of the SNN exploits an important characteristic of images, namely, the fact that in any given image over a period of time, the diversity of objects is quite limited~\cite{farhadi2019tkd}, and therefore, a DNN may not be necessary and a smaller, shallower model will suffice. On the other hand, when changes do occur, they must be detected, and the shallow model must be updated.  Our approach detects such changes, activates the DNN as required, which in turn transfers the new knowledge (the encoding of the ground truth in the new weights) from the edge device to the user-end device to update the shallow model, all while performing inference, i.e., at run-time. The knowledge transferred includes the weights of the CNN in the decoder layers (layers that detect the objects using the extracted features from previous layers). This transfer enables us to improve the inference time of object detection while maintaining the accuracy of deep model.  

We demonstrate these ideas by implementing the proposed approach on a pair of devices where the user-end device is an NVIDIA Jetson Nano development kit and the edge device is a Dell workstation with NVIDIA Titan Xp GPU. The experiments show that the proposed method can achieve the desired accuracy while having a significantly lower inference time. Moreover, total energy consumption of the user-end device was reduced by \textbf{78\%} when compared to running the DNN entirely on the user-end device. 


The main contributions of this paper are as follow:
\begin{itemize}
    \item We demonstrate a novel computational framework for transferring knowledge between two devices, one executing a DNN, and the other executing an SNN. This approach substantially advances edge computing for perform very complex and computationally intensive applications. 
    \item We present an extensive exploration of various ways in which the knowledge transfer can take place, and evaluate them in terms of specific, well defined and appropriate metrics. 
    \item The quality of the detection results depends on when the DNN should be activated for possible knowledge transfer.  Toward this, we present an novel \textit{key-frame} selection mechanism that substantially improves the efficiency of the knowledge transfer. 
    \item The proposed framework for incremental learning in object detection is made open-source and will be released for public distribution on Github. 
\end{itemize}
The rest of this paper is organized as follows: Section \ref{related} summarizes the background and related work which has been done previously. In Section \ref{approach}, the proposed approach using edge computing has been proposed. The experimental platform and the results are illustrated in Section \ref{results}. Ultimately, the conclusions are drawn in Section \ref{conclusion}. 
